Higgs Physics at the CLIC Electron-Positron Linear Collider

The Compact Linear Collider (CLIC) is an option for a future e+e- collider operating at centre-of-mass energies up to 3 TeV, providing sensitivity to a wide range of new physics phenomena and precision physics measurements at the energy frontier. This paper is the first comprehensive presentation of the Higgs physics reach of CLIC operating at three energy stages: sqrt(s) = 350 GeV, 1.4 TeV and 3 TeV. The initial stage of operation allows the study of Higgs boson production in Higgsstrahlung (e+e- -> ZH) and WW-fusion (e+e- -> Hnunu), resulting in precise measurements of the production cross sections, the Higgs total decay width Gamma_H, and model-independent determinations of the Higgs couplings. Operation at sqrt(s) > 1 TeV provides high-statistics samples of Higgs bosons produced through WW-fusion, enabling tight constraints on the Higgs boson couplings. Studies of the rarer processes e+e- -> ttH and e+e- -> HHnunu allow measurements of the top Yukawa coupling and the Higgs boson self-coupling. This paper presents detailed studies of the precision achievable with Higgs measurements at CLIC and describes the interpretation of these measurements in a global fit.

==> Main/packages.tex <==
%\usepackage{titlepage}

\usepackage{lipsum}

\RequirePackage[T1]{fontenc}

\smartqed  % flush right qed marks, e.g. at end of proof

%\usepackage{draftwatermark}
%\SetWatermarkFontSize{1.8cm}
%\input{globalrevision.tex}

\RequirePackage{color}
\RequirePackage{graphicx}
\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
\RequirePackage{feynmp}
\RequirePackage{amsmath}
\RequirePackage{heppennames2}
\RequirePackage[numbers,sort&compress]{natbib}

\usepackage{bm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{tocloft}
\usepackage{texnames}
\usepackage[T1]{fontenc}
\pagestyle{plain}
\usepackage{color}
\usepackage{wasysym}

%\usepackage[square,numbers,sort]{natbib}
\usepackage{url}

%\usepackage{draftwatermark}
%\SetWatermarkFontSize{1.8cm}

\usepackage{units}
\usepackage{siunitx}
\usepackage{booktabs}
\usepackage{subfig}
\usepackage{graphicx}
\usepackage{feynmp}
\DeclareGraphicsRule{*}{mps}{*}{}


%For tables
\usepackage{multirow}

%%For title layout
\usepackage{textpos} % for placement of logo 
\usepackage{relsize} 

%%Font treatment
\usepackage{mathptmx}
\usepackage[scaled=.90]{helvet}
\usepackage{courier}
\usepackage[T1]{fontenc} %font enconding
\usepackage[latin9]{inputenc} %input encoding


%%Layout spacing

% align left the itemize and enumerate lists, and reduce space
\usepackage{enumitem}
\setlist{noitemsep}
\setlist[itemize]{leftmargin=*, topsep=-2pt, partopsep=0pt, itemsep=2pt}
\setlist[enumerate]{leftmargin=*, topsep=0pt, partopsep=0pt, itemsep=0pt}

% no paragraph indentation
\setlength{\parindent}{0pt}
\setlength{\parskip}{1.3ex} % less space between paragraphs


% hyper ref and cleverer needs to be last
\RequirePackage[colorlinks,breaklinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}
\renewcommand*{\sectionautorefname}{Section}
% \hypersetup{draft}
\urlstyle{same}
% fix bug in svjour3 (only happens with cleverer)
\makeatletter
%\def\cl@chapter{\cl@chapter \@elt {theorem}}%bug in class
\def\cl@chapter{\@elt {theorem}}
\makeatother

\let\subsectionautorefname\sectionautorefname
\let\subsubsectionautorefname\sectionautorefname

\RequirePackage[capitalize]{cleveref}


%============================================%
% Additional units and configuration
%============================================%
\sisetup{
  separate-uncertainty=true, % write 5.3+-0.2 instead of 5.3(2)
  range-phrase=--,           % write 1--100 instead of 1 to 100
  range-units=single,        % write 1--100 GeV instead of 1 GeV -- 100 GeV
}

\DeclareSIUnit\micron{\micro\metre}
\DeclareSIUnit\rad{\radian}
\DeclareSIUnit\mrad{\milli\radian}
\DeclareSIUnit\gauss{G}
\DeclareSIUnit\eVperc{\eV\per\clight}
\DeclareSIUnit\nanobarn{\nano\barn}
\DeclareSIUnit\picobarn{\pico\barn}
\DeclareSIUnit\femtobarn{\femto\barn}
\DeclareSIUnit\attobarn{\atto\barn}
\DeclareSIUnit\zeptobarn{\zepto\barn}
\DeclareSIUnit\yoctobarn{\yocto\barn}
\DeclareSIUnit\nb{\nano\barn}
\DeclareSIUnit\pb{\pico\barn}
\DeclareSIUnit\fb{\femto\barn}
\DeclareSIUnit\ab{\atto\barn}
\DeclareSIUnit[number-unit-product = {}] \percent{\%} % remove space between number and percent sign

%%% Local Variables: 
%%% mode: latex
%%% TeX-PDF-mode: t 
%%% TeX-master: "../clicsnowmass"
%%% End: 

